Extreme Low-State Quantized Transformer for Electricity-Load Forecasting

Aggressive low-state weight quantization can substantially reduce neural-network representational flexibility, making predictive performance difficult to preserve when only a few discrete weight states are available. We investigate this regime for Transformer-based electricity-load forecasting using 3-, 5-, 7-, and 16-state weight quantization across feed-forward-only and attention-plus-feed-forward quantization. Two tasks predict either the next hour or the next 24 hours from the preceding 48 hours across two co-primary electricity-consumption datasets. Direct post-training quantization (PTQ) increased mean normalized root-mean-square error (NRMSE) relative to full precision by 6.25 and 7.04 percentage points in Datasets A and B, whereas quantization-aware fine-tuning (QAT-FT) recovered approximately 90.2% and 94.5% of these penalties. Quantization-aware training from random initialization (Scratch-QAT) also produced competitive low-state solutions, with particularly favorable behavior at three states. We further introduce accumulated-update thresholding, which accumulates optimizer-proposed weight changes before commitment. Relative to paired Scratch-QAT controls, this reduced committed shadow-weight updates by approximately 99.7% and discrete state transitions by approximately 77--80%, while mean NRMSE changed by only +0.042 and +0.197 percentage points. These results show that useful Transformer forecasting can be retained under highly discrete weight representations while strongly suppressing target-state activity, supporting a prospective route toward compact, low-activity edge forecasting using multilevel synaptic devices.

==> tables/table_config_structure.tex <==
\begin{table}[t]
\centering
\caption*{Table 1b. Chronological development, selection, and final evaluation structure}

\small
\begin{tabularx}{\textwidth}{
    @{}
    p{0.20\textwidth}
    p{0.12\textwidth}
    p{0.27\textwidth}
    p{0.13\textwidth}
    X
    @{}
}
\toprule
Stage &
Dataset &
Configuration structure &
Count &
Scientific role \\
\midrule

Broad quantization development &
Dataset A &
3 series $\times$ 2 horizons $\times$ 2 locations $\times$ 11 state counts &
132 base combinations &
Explore the quantization regime during development \\

Three-fold development evaluation &
Dataset A &
132 combinations $\times$ 3 expanding-window folds &
396 fold-specific evaluations &
Development-stage comparison and method selection \\

Frozen Dataset-A configuration space &
Dataset A &
3 series $\times$ 2 horizons $\times$ 2 locations $\times$ 4 selected state counts &
48 configurations &
Final protocol after selection of 3, 5, 7, and 16 states \\

Untouched Dataset-A final evaluation &
Dataset A &
Same 48 frozen configurations &
48 configurations &
Final evaluation after retraining on the frozen final training period \\

Frozen methodological transfer &
Dataset B &
1 series $\times$ 2 horizons $\times$ 2 locations $\times$ 4 selected state counts &
16 configurations &
Evaluate the Dataset-A-frozen methodology without Dataset-B-specific reselection \\

Final cross-dataset evidence matrix &
Datasets A + B &
48 Dataset-A + 16 Dataset-B configurations &
64 configurations &
Structured paired evidence used for the principal cross-dataset analyses \\

\bottomrule
\end{tabularx}
\end{table}
